SCL with Theory Constraints

We lift the SCL calculus for first-order logic without equality to the SCL(T) calculus for first-order logic without equality modulo a background theory. In a nutshell, the SCL(T) calculus describes a new way to guide hierarchic resolution inferences by a partial model assumption instead of an a priori fixed order as done for instance in hierarchic superposition. The model representation consists of ground background theory literals and ground foreground first-order literals. One major advantage of the model guided approach is that clauses generated by SCL(T) enjoy a non-redundancy property that makes expensive testing for tautologies and forward subsumption completely obsolete. SCL(T) is a semi-decision procedure for pure clause sets that are clause sets without first-order function symbols ranging into the background theory sorts. Moreover, SCL(T) can be turned into a decision procedure if the considered combination of a first-order logic modulo a background theory enjoys an abstract finite model property.

==> paper-dpll.tex <==
%!TEX root = paper

%%% Local Variables:
%%% mode: latex
%%% TeX-master: "paper"
%%% End:

\section{Alternative Completeness}

Suppose we are in a DPLL-like scenario where we only propagate by conflict without learning. Our rules would be modified as:

%\bigskip
%\shortrules{Propagate}
%{$(M;N;U;k;\top)$}
%{$(M, L\cdot\sigma^{\Lambda\| C\lor L};N;U;k;\top)$}
%{provided $\Lambda\| C\lor L\in (N\cup U)$, $C\sigma$ is ground and false under
%	$M$, $\Lambda\sigma$ is ground and true, and $L\sigma$ is undefined in $M$}{\SCL}{12}

\bigskip
\shortrules{Decide}
{$(M;N)$}
{$(M,\Delta\|L^\dagger;N)$}
{provided $\Delta\|L$ is a ground constrained literal \st $M\not\models\Delta\|L$ and $M\not\models\lnot(\Delta\|L)$}{\SCL}{12}

\bigskip
\shortrules{Backtrack}
{$(M,\Delta\|L^\dagger,M';N)$}
{$(M, e_1\|\bot,\dots, e_n\|\bot, \comp(L);N)$}
{provided there are no decision literals in $M'$ and $M,\Delta\|L^\dagger,M'\models \lnot (\Delta'\|D)$ for a constrained clause $\Delta'\|D$ in $N$ and $\Delta = e_1\land\dots\land e_n$.}{\SCL}{11}

\bigskip
As a sanity test we should be able to combine Decide and Backtrack to obtain a something similar to a Propagate.

\[N = \{ x \approx 1 \| P(x), x \approx 2 \| Q\lor P(x), x \approx 3 \|Q\lor  P(x), Q\lor Q,x\approx 2 \land x \approx 3\| \lnot P(x) \lor\lnot P(y)\}\]




\bigskip
\shortrules{Abstract}
{$N\uplus \{\Lambda\|C\lor L(t_1,\ldots,t_n)\}$}
{$N\uplus \{\Lambda\land t_i\approx z \|C\lor L(t_1,\ldots,t_n)[z]_i\}$}
{provided $1\le i\le n$, $t_i$ is a pure background term not already a variable, and $z$ is a fresh variable of sort $S$.}{ABSTR}{11}



==> paper-examples.tex <==
%!TEX root = paper

%%% Local Variables:
%%% mode: latex
%%% TeX-master: "paper"
%%% End:


\begin{example}
  [counterexample]
  Consider an unsatisfiable clause set $N = \{D_1,D_2,D_3,D'\}$
  where $D_i \equiv x \approx i \| P(x)$
  and $D' \equiv x\approx 2 \land x \approx 3\| \lnot P(x) \lor\lnot P(y)$.
  A regular run could get stuck if the first propagation is $D_1$.

  Another case is \[N = \{ x \approx 1 \| P(x), x \approx 2 \| Q\lor P(x), x \approx 3 \|Q\lor  P(x), Q\lor Q,x\approx 2 \land x \approx 3\| \lnot P(x) \lor\lnot P(y)\}\]

\end{example}

\begin{definition}[New Strategy]
	We instantiate propagations with new constants if and only if propagations with old constants are exhausted. Similarly for decisions (Conflicts can always be instantiated with old constants(?))
\end{definition}

the example above would thus become

\[
\begin{aligned}
	(N;\top;&0;\epsilon)\\
	(N;\top;&0;c_1=1\|[P(c_1)])\\
	(N;\top;&0;c_1=1\|[P(c_1)],c_2=2\|[P(c_2)])\\
	(N;\top;&0;c_1=1\|[P(c_1)],c_2=2\|[P(c_2)],c_3=3\|[P(c_3)])\\
\end{aligned}
\]

\begin{example}
	A given clause $C$ can have more than one propagated literal on the trail:\[N=\{P(x)\lor Q(x), \lnot P(a), \lnot Q(b)\}\]
	creates the trail $[\lnot P(a), \lnot Q(b), Q(a), P(b)]$ by propagation.
\end{example}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\section{TODO List}
\begin{itemize}
\item regular runs on well formed states preserve strong consistency
\item 
\end{itemize}


==> paper-hires.tex <==
In this paper we replace the ordering restrictions of hierarchic superposition
by the selection of inferences through an explicit partial model assumption. Furthermore, we do not
consider equality in the free part.
In this case the inference rules of hierarchic superposition simplify to hierarchic resolution inferences.
First, we define the hierarchic resolution calculus that
is an instance of hierarchic superposition without equality and ordering restrictions on the inferences~\cite{BachmairGanzingerEtAl94}.

\bigskip
\shortrules{Hierarchic Resolution}{$(N\disjun\{\Lambda_1\| C_1 \lor P(\tenum{t}{n}), \Lambda_2\| C_2 \lor \neg P(\tenum{s}{n})\})$}{$N\cup\{\Lambda_1\| C_1 \lor P(\tenum{t}{n}), \Lambda_2\| C_2 \lor \neg P(\tenum{s}{n})\}\cup\{(\Lambda_1, \Lambda_2\| C_1 \lor C_2)\sigma\}$}{where $\sigma$ is the mgu of  $P(\tenum{t}{n})$  and $P(\tenum{s}{n})$ and $\sigma$  is simple}{HRES}{30}

\bigskip
\shortrules{Hierarchic Factoring}{$(N\disjun\{\Lambda\| C \lor L \lor K)\})$}{$N\cup\{\Lambda\| C \lor L \lor K\}\cup\{(\Lambda\| C \lor L))\sigma\}$}{where $\sigma$ is the mgu of  $L$  and $K$ and $\sigma$  is simple}{HRES}{30}

In the hierarchic superposition context factoring is defined on positive literals only. Here, we include negative literals
as well. Of course, this does not affect soundness nor completeness.

\Todo{Maybe we should define compact theories.}
\begin{definition}[Compact Theories] \label{prelim:def:compact}
A (background) theory $\theory^{\bspec} = (\sig^{\bspec}, \modset^{\bspec})$ is compact if every infinite set of $\sig^{\bspec}$-clauses that is inconsistent relative to $\modset^{\bspec}$ has a finite subset that is also inconsistent relative to $\modset^{\bspec}$.\Todo{Should we call them pure $\sig^{\bspec}$-clauses although this might cause confusion with pure clause sets?}
\end{definition}

\begin{corollary}[Completeness of Hierarchic Resolution~\cite{BachmairGanzingerEtAl94}]
If the background theory is compact then $\Rightarrow_{\text{HRES}}$ is complete for pure clause sets.
\end{corollary}


\begin{lemma}[$\SCLT$ Simulates Hierarchic Resolution] \label{lemm:simres-resolve}
  Let $N$ be a constrained clause set, $\Lambda\|C\lor P(x_1\ldots,x_n)$ and
  $\Delta\| D\lor \neg P(y_1,\ldots,y_n)$ be non-redundant constrained clauses in $N$
  % such that $C$ and $D$ are non-empty
  ,
  $\eta=\mMGU(P(x_1\ldots,x_n), P(y_1,\ldots,y_n))$,
  % the literals $P(x_1\ldots,x_n)$ and $P(y_1,\ldots,y_n)$ are not duplicated in either $C$ or $D$
  and the clause $(\Lambda\land \Delta\|C\lor D)\eta$ is not redundant.
  Let $C_0 = C\eta \setminus P(x_1\ldots,x_n)\eta$ and $D_0 = D\eta \setminus P(x_1\ldots,x_n)\eta$
  then, there is a regular $\SCLT$ run starting from the state
  $(\epsilon;N;\emptyset;B;0;\top)$ where the clause $(\Lambda\land \Delta\|C_0\lor D_0)\eta$ is learned,  made redundant, or $C_0\lor D_0$ is the empty conflict clause at the end of a conflict resolution,
  provided $B$ contains sufficiently many foreground constants.
\end{lemma}
\begin{proof}
  We assume clauses in $N$ are variable disjoint.
  Let $\theta$ be a grounding substitution on the variables of
  $(\Lambda\|C\lor      P(x_1,\ldots,x_n))\eta$ and
  $(\Delta \|D\lor \neg P(y_1,\ldots,y_n))\eta$
  such that distinct literals are mapped to distinct
  ground literals. This requires at most
  $|\vars(\Lambda\|C\lor P(x_1\ldots,x_n))| + |\vars(\Delta\| D\lor \neg P(y_1,\ldots,y_n))| - n$
  different foreground constants.
  Let $\{L_1,\ldots,L_n\} = (C \lor D)\eta\theta \setminus  P(x_1,\ldots,x_n)\eta\theta = (C_0 \lor D_0)\eta\theta $.
  For all clauses $\Gamma'\| C'\in (N\cup U)$ such that
  $C'\rho \subset (C\lor P(x_1\ldots,x_n))\eta\theta$ or
  $C'\rho \subset (D\lor \neg P(y_1\ldots,y_n))\eta\theta$ or
  $C'\rho \subset (\Lambda\land \Delta\|C\lor D)\eta\theta$
  we build a constraint $\Gamma\rho$ such
  that $\Gamma\rho \models \neg(\Gamma'\rho)$
  for all $\Gamma'\| C'$ and
  $\Lambda\eta\theta\land\Delta\eta\theta\land\Gamma\rho\land\adiff(B)$ is satisfiable.
  If this cannot be constructed using a sufficiently
  large set $B$ then one of the clauses
  $\Lambda\|C\lor P(x_1\ldots,x_n)$,
  $\Delta\| D\lor \neg P(y_1,\ldots,y_n)$,
  $(\Lambda\land \Delta\|C\lor D)\eta$
  is redundant, because the $\Gamma'\| C'$
  are all strictly smaller than their counterparts.
  Note that we are implicitly using here a subset ordering which is contained
  in the reduction ordering considered by hierarchic resolution (superposition).

  We can start our derivation with $n$ Decisions
  and adding the respective background literals
  where at the $i$-th step we decide the literal
  $K_i=\comp(L_i)$ to obtain via a regular run the state\newline
  \centerline{$(K_1^1,\Lambda'\eta\theta,\Delta'\eta\theta, \Gamma\rho, M_1,K_2^2,M_2,K_3^3,M_3,\ldots,K_n^n; N;U;B;n;\top),$}
  $K_i = \comp(L_i)$
  where $\Lambda'\eta\theta,\Delta'\eta\theta$ are the constraints of the two clauses instantiated by $\eta\theta$ without (common) duplicates,
  and the $M_i$ contain potentially propagated literals. Here at most $|\vars(N\cup U)|\times n$ different constants from $B$ are needed.
  If there is a conflict possible already before reaching $K_n^n$ where the conflict clause
  contains literals other than $\{L_1,\ldots,L_n\}$ we apply conflict resolution with a restart. This can only happen finitely often, because
  every generated trail is a subtrail of the trail above with respect to the $K_i$ and $\Lambda'\eta\theta,\Delta'\eta\theta, \Gamma\rho$ and there are
  only finitely many such subtrails. If there is a conflict possible already before reaching $K_n^n$ where the conflict clause is build from
  literals $\{L_1,\ldots,L_n\}$ this is a contradiction to our construction of $\Gamma\rho$.

  For otherwise when reaching $K_n^n$, the literal $P(x_1\ldots,x_n)\eta\theta$ is still undefined but every other literal
  in $C_0\eta\theta$ is falsified under the current trail;
  so in the next step we can propagate $P(x_1\ldots,x_n)\eta\theta$ on
  the trail and obtain.\newline
  \centerline{$(M, P(x_1\ldots,x_n)\eta\theta^{\Lambda\|C_0\lor P(x_1\ldots,x_n)\cdot\eta\theta},\Lambda\eta\theta,;
    N;\emptyset;B;n;\top),$}
  where $M = K_1^1,\Lambda'\eta\theta,\Delta'\eta\theta, \Gamma\rho, M_1,K_2^2,M_2,K_3^3,M_3,\ldots,K_n^n$,
  and $C_0$ is the clause obtained by removing the exact duplicates of $P(x_1\ldots,x_n)\eta$ from $C$.
  Now the rule Conflict is applicable to
  $\Delta\|(D \lor \neg P(y_1,\ldots,y_n))\eta\theta$ resulting in\newline
  \centerline{$(M,P(x_1\ldots,x_n)\eta\theta^{\Lambda\|C_0\lor P(x_1\ldots,x_n)\cdot\eta\theta},\Lambda\eta\theta;
    N;\emptyset;B;n;
    \Delta\|D\lor \neg P(y_1,\ldots,y_n)\cdot \eta\theta).$}
  We can now apply Factorize on all duplicates of $\lnot P(x_1\ldots,x_n)\eta\theta$ in $D$
  to obtain the conflict clause $\Delta\|D_0\lor \neg P(y_1,\ldots,y_n)\cdot \eta\theta$,
  Skip enough times to reach the literal $P(x_1\ldots,x_n)\eta\theta^{\Lambda\|C_0\lor P(x_1\ldots,x_n)\cdot\eta\theta}$
  and then  Resolve once to reach the state\newline
  \centerline{$(M;N;\emptyset;B;n; (\Lambda\land\Delta\|C_0\lor D_0)\eta\cdot\theta).$}
  From this state we can finally backtrack and
  learn $(\Lambda\land\Delta\|C_0\lor D_0)\eta$.
\end{proof}


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%




%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\begin{theorem}\label{theo:sim-hsup}
  Starting with a sufficiently large set of constants $B$, $\SCLT$
  can simulate a hierarchic resolution proof by a regular run.
\end{theorem}
\begin{proof}%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%lang comp reprudacbility topic+result+ibteresting+relevant originaloty
  By Lemma~\ref{lemm:simres-resolve}
  $\SCLT$ can simulate a single application of hierarchic resolution.
  Now a hierarchic resolution proof may actually also contain
  hierarchic factoring steps, we show that given two constrained clauses $\Lambda\|C\lor P(x_1,\ldots,x_s)$ and $\Delta\|D\lor\lnot P(y_1,\ldots,y_s)$
  we can simulate any number of hierarchic factorization steps on them, producing clauses $\Lambda''\|C''\lor P(x_1,\ldots,x_s)$ and $\Delta''\|D''\lor\lnot P(y_1,\ldots,y_s)$ respectively,
  followed by a hierarchic resolution step
  producing a clause $\Lambda'\Delta'\|C'\lor D'$ can be integrated in the simulation of resolution used in Lemma~\ref{lemm:simres-resolve}.

  Let $N$ be a constrained clause set,
  $C_0 = \Lambda\|C\lor      P(x_1,\ldots,x_sn)$ and
  $D_0 = \Delta \|D\lor \neg P(y_1,\ldots,y_s)$ be constrained clauses in $N$,
  let $C_1,\ldots,C_n$ and $D_1,\ldots,D_m$ be sequences of clauses such that $C_i$ ($D_j$) is the result of
  applying a hierarchic factorization to $C_{i-1}$ ($D_{j-1}$) for $1\le i\le n$ ($1\le j\le n$),
  let $\rho_i$ and $\rho'_j$ be the unifier used in the factorizations that produced $C_i$ and $D_j$ respectively,
  let $\rho = \rho_1\dots\rho_n\rho'_1\dots\rho'_m$,
  let $\Lambda'\land\Delta'\|C'\lor D'$ be the resolvent of
  $C_n = \Lambda''\|C''\lor       P(x_1,\ldots,x_s)$ and
  $D_m = \Delta'' \|D''\lor \lnot P(y_1,\ldots,y_s)$
  let $\eta = \mMGU(P(x_1,\ldots,x_s),P(y_1,\ldots,y_s))$
   and let $\theta$ be a grounding substitution that maps distinct variables in $C_n\rho\eta, D_n\rho\eta$
  to distinct constants.

  %For every literal $L_i$ in $C_n\cup D_n = \{L_1,\dots,l_h\}$ we define a set $A_i$ of literals in $C_0\cup D_0$
  % We show that we can simulate this kind of inference. Each of the factorization applied introduces an $\mMGU$ of two literals of $C_i$ or $D_j$, let be the unifier used in the factorization that produces and $\eta = \mMGU(P(x_1,\ldots,x_s),P(y_1,\ldots,y_s))$, Finally we consider a grounding substitution and the clause $(\Lambda\land \Delta\|C\lor D)\eta$ is not redundant. We show that such a sequence of factorization and resolution steps can be simulated by $\SCLT$.

  We proceed with the conflict search phase as in the proof of Lemma~\ref{lemm:simres-resolve},
  Eventually we either make the resolvent $\Lambda'\land\Delta'\|C'\lor D'$ redundant or we obtain a state
  {$(M,P(x_1\ldots,x_n)\rho\eta\theta^{\Lambda\|C_0'\lor P(x_1\ldots,x_n)\cdot\rho\eta\theta},\Lambda\rho\eta\theta;
    N;U;B;n;\Delta\|D\lor \neg P(y_1,\ldots,y_n)\cdot\rho\eta\theta)$}
  where $C_0'$ is $C$ where all copies of $P(x_1\ldots,x_n)\rho\eta\theta$ have been removed. By construction these
  are all literals that were factorized in the original construction.

  Now we note that two ground literals in $\Delta\|D\lor \neg P(y_1,\ldots,y_n)\cdot\rho\eta\theta$
  are equal if and only if they were factorized in the original construction, so we can simply apply
  factorization eagerly. After all factorizations have been applied, we can resolve once to obtain
  the conflict clause $\Lambda\land\Delta''\|C_0'\lor D'' \cdot\rho\eta\theta$.
  Again we can note that in the current conflict clause there are duplicated literals
  if and only if they correspond to factorized literals of the original construction,
  so we can apply factorization eagerly and finally obtain the conflict clause
  $\Lambda'\land\Delta'\|C'\lor D'\cdot\rho\eta\theta$, from which we can backtrack to learn our desired clause.
\end{proof}





%%% Local Variables:
%%% mode: latex
%%% TeX-master: "paper"
%%% End:

